Receptive Field Regularization Techniques for Audio Classification and Tagging with Deep Convolutional Neural Networks

In this paper, we study the performance of variants of well-known Convolutional Neural Network (CNN) architectures on different audio tasks. We show that tuning the Receptive Field (RF) of CNNs is crucial to their generalization. An insufficient RF limits the CNN's ability to fit the training data. In contrast, CNNs with an excessive RF tend to over-fit the training data and fail to generalize to unseen testing data. As state-of-the-art CNN architectures-in computer vision and other domains-tend to go deeper in terms of number of layers, their RF size increases and therefore they degrade in performance in several audio classification and tagging tasks. We study well-known CNN architectures and how their building blocks affect their receptive field. We propose several systematic approaches to control the RF of CNNs and systematically test the resulting architectures on different audio classification and tagging tasks and datasets. The experiments show that regularizing the RF of CNNs using our proposed approaches can drastically improve the generalization of models, out-performing complex architectures and pre-trained models on larger datasets. The proposed CNNs achieve state-of-the-art results in multiple tasks, from acoustic scene classification to emotion and theme detection in music to instrument recognition, as demonstrated by top ranks in several pertinent challenges (DCASE, MediaEval).

==> a6_futher_mediaeval.tex <==
\label{app:further:mediaeval}

\khaled{ includes shake-shake and FA, Not sure if they fit the story any thoughts?}
Figures~\ref{fig:openmic:main:prauc} shows the PR\_AUC of CP\_ResNet variants on  MediaEval-MTG-Jamendo. We see that both filter-damping (ERF-regularization) and shake-shake regularization counters the overfitting caused by the increasing the Max RF, in comparison to CP\_ResNet and CP\_DenseNet (Figure\ref{fig:mediaeval:main:acc}) and CP\_FAResNet.
\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/app_meidaeval_acc_all.pdf}
\caption{Testing PR\_AUC of CP\_ResNet variants on  MediaEval-MTG-Jamendo   (Emotion and theme recognition in Music task in MediaEval 2019). SS: shake-shake regularization}
\label{fig:openmic:main:prauc}
\end{figure}

==> a7_furhter_openmic.tex <==
\label{app:further:openmic}


\khaled{ includes shake-shake and FA, Not sure if they fit the story any thoughts?}
Figures~\ref{fig:openmic:main:prauc} shows the F-Score of CP\_ResNet variants on the testing set of  OpenMIC. We see that both filter-damping (ERF-regularization) and shake-shake regularization counters the overfitting caused by the increasing the Max RF, in comparison to CP\_ResNet and CP\_DenseNet (Figure\ref{fig:mediaeval:main:acc}) and CP\_FAResNet.
\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/app_opemic_fscore_damp.pdf}
\caption{Testing F-Score of CP\_ResNet variants on  OpenMIC. SS: shake-shake regularization}
\label{fig:openmic:main:prauc}
\end{figure}

==> old_s1_intro.tex <==

\IEEEPARstart{C}onvolutional Neural Networks (CNNs) have come to dominate many domains~\cite{LIU201711survey}, including image classification~\cite{krizhevsky2012imagenetalex}, 
% audio classification~\citep{cite}, speech recognition~\citep{cite}.
% The recent success started in an image classification task~\cite{krizhevsky2012imagenetalex} in computer vision. 
% The success of CNNs followed shortly in different fields such as 
natural language processing~\cite{shen2014learning,kim-2014-convolutional,collobert2014deepcnnmultitask}, and 
speech recognition~\cite{hinton2012cnnspeach}.
% \khaled{some connection}
In computer vision, CNNs have shown to perform better with deeper architectures~\cite{simonyanVeryDeepConvolutional2014,heDeepResidualLearning2016,huangDenselyConnectedConvolutional2017}.
Following this trend, many researchers working on audio tagging and classification tasks have started to employ such deep architectures from vision, by extracting image-like features such as spectrograms~\cite{lee2009speccnn,eghbal-zadehCPJKUSubmissionsDCASE20162016,hersheyCNNArchitecturesLargescale2017}.

In this work, we will show that using deeper architectures which have proven successful in vision tasks, does not necessarily guarantee good performance in audio tasks.
% this doesn't hold in general for different computer listening tasks.
In particular, we show that deep CNNs designed for vision often have a large Receptive Field (RF) that is not suitable for 
audio processing tasks, and such models fail to generalize.
We provide solutions to this problem by regularizing the RF of different variants of deep architectures,
and we demonstrate that this massively improves results in various audio classification and tagging tasks.\footnote{In fact, using our proposed RF regularized architectures, we have achieved top ranks in several international challenges on different tasks~\cite{Koutinitrrfcnns2019,koutini2019emotion}\gerhard{also mention DCASE2020?}\khaled{i think we should mention it in low complexity settings}}
We portray the RF of CNNs as an important hyper-parameter and design factor %\hamid{design choice does not fit very well here.} 
that should be carefully tuned and investigated, when adapting a CNN architecture (which has been designed in other domains such as vision)
% \footnote{We analyze CNN architectures that operate on spectrograms as input.})
to the audio world. 

Moreover, 
% we use these results to 
we provide \textit{generic and systematic approaches} to controlling the RF of a CNN architecture.
% \gerhard{This should perhaps be stressed more strongly in the abstract}
% , and we propose template \hamid{suggestion: several} CNN architectures \hamid{that have been} 
Using this method, we will show how well-known vision architectures can be effectively adapted to the audio domain.
% that uses 
%using a single 
% introduced
%hyper-parameter that controls the RF of the CNN.
 
We will demonstrate the effectiveness of our approaches by performing large-scale experiments on three different audio classification and tagging tasks, and using several datasets.
%\hamid{What do you mean in the next sentence?}
We study the common components that are usually used to build CNNs %, such as grouped, dilated convolutional layers etc.,
and demonstrate their effect on the RF. % and therefore the generalization of CNNs. 
Furthermore, we perform experiments to investigate the individual impact of these components on the performance of CNNs.



% \hamid{instead of:}We differentiate between the impact of the RF over the time and over the frequency dimensions.
% We study different RF setups over the both dimension and their combined effect on the generalization of CNNs. 
More specifically, we study the effect of RF regularization over the time and the frequency dimensions, individually and jointly, and how the RF size over these dimensions affects the generalization of CNNs.
% \gerhard{this it getting too long ...}
% The experimental results show that tuning the RF over the frequency dimension has a higher impact than the time dimension. On the one hand, CNNs with too small RF over either of the dimension under-fit and therefore degrade in performance. On the other hand, CNNs with too large RF on either dimensions both tend to overfit on the training data and degrade in performance on unseen testing sets. Nevertheless, the results show that the performance is more sensitive to the RF size over the frequency dimension.
Generally, the experimental results will show that the performance is more sensitive to the RF size along the frequency dimension than on time.

%\hamid{the rest of the paragraph is inconclusive. Try to state it better.}

% \hamid{the next paragraph might have too many detail for the intro. Maybe you can sort of merge it with the previous paragraph, and write the punch line?}
As an additional important dimension, we differentiate between (a) the \textit{Maximum Receptive Field} of a CNN, which can be calculated from studying its architecture, and (b) the \textit{Effective Receptive Field}~\cite{luoUnderstandingEffectiveReceptive2016} (ERF) of a trained CNN. % which is a function of ....... . 
We introduce a measure for the ERF and analyse the difference to the maximum RF. 
%We also introduce a systematic method to control the ERF of a CNN without changes to the topology or the filters the network We call it \textit{damping}, and again study the effect of controlling the ERF over both dimensions. 
Finally, we introduce a novel method we call \emph{filter damping}, that enables us to control the ERF of a CNN, without changing the architectural topology, or the filters the network. We show that filter damping will improve generalisation of models, and will adapt the ERF of models to better fit the task at hand.

The remainder of the paper is structured as follows. After a brief discussion of the related work (Section \ref{sec:related_work}) and presentation of the acoustic tasks and the data sets we have chosen for our investigations (Section \ref{sec:tasks_datasets}), Section \ref{sec:rf_cnns} takes a closer look at the concepts of maximum and effective receptive field, and proposes ways to determine and measure them in a given model. 
The presentation of our proposed principled methods for controlling RF in various deep CNN architectures, and the corresponding experimental investigations, will then be split into two strands: Sections \ref{sec:control_max_rf} and \ref{sec:results} focus on the maximum RF, while Sections \ref{sec:control_erf} and \ref{sec:result_erf} will be discussing the ERF. We explain the setup we use to perform the experiments in Appendix~\ref{app:exp_setup}.  
Finally, the additional experimental results that focus on the influence of a particular component of CNNs, will be presented in  Appendix~\ref{app:arch:design:components:maxrf}.


==> omited_s8_fa_cnn.tex <==
% \label{sec:fa_cnn}


% Some tasks require the internal representation of the CNN to be frequency sensitive ... \hamid{motivate FA: ...since RF regularisation limits the rf of CNNs, ...}
 
%  \khaled{rewrite:}\cite{koutinifaresnet2019}

% In CNNs that have a large enough RF, deeper convolutional layers can infer the frequency information of their input feature maps. However, CNNs with large RF degrade in performance and fail to generalize in acoustic scene classification as shown in~\cite{Koutini2019Receptive}.
% On the other hand, in high-performing fully convolutional CNNs, learned CNN filters are agnostic to the frequency range information of the feature maps. In other words, the spectrograms and feature maps can be rolled over both the time and frequency dimension with a minor impact on the network predictions. This is one side effect of limiting the receptive field of CNNs on spectograms. %is that convolutional layers have less inferred information about the frequency context of the feature maps. In addition to that, 
% We propose a new convolutional layer, which we call \emph{Frequency-aware Convolution}, to make filters aware and more specialized in certain frequencies by concatenating a new channel containing the frequency information of each spatial pixel to each feature map. This technique is similar to CoordConv~\cite{liu2018intriguing}, where the network input is padded with the pixels' coordinates. In our case, we pad all feature maps with a real number indicating the frequency context of each pixel.\footnote{In this paper, we used a number between $-1$ and $1$, where $-1$ represents the lowest and $1$ the highest frequency in the spectrogram. But this range can be adapted according to the value range of the input.}


% The CNN models that incorporate our frequency-aware layer will be called the \emph{Frequency-Aware Convolutional Neural Networks (FACNNs)}. Similarly, we call the frequency-aware ResNet \emph{FAResNet}.
% We denote the value of the pixel with spatial index $(f,t)$ in the new channel as $V(f,t)$; it is calculated as
% \begin{equation}
%   \label{eqn:locpad}
%     V(f,t)=f/F
% \end{equation}
% where $F$ is the size of the frequency dimension of the feature map, $f$ is the pixel index in the frequency dimension, and $t$ is the pixel index in the time dimension.
% This new channel gives the convolutional filters a frequency context.

% Since making CNNs frequency-aware (by adding the new channel) does not alter the maximum RF of the network, we control the maximum RF of FAResNets similar to ResNet (Section~\ref{sec:resnet}) by changing $\rho$.
 	

==> ommited_a1_maxrf_withpooling.tex <==
\label{app:maxrf:traintest:pooling}

In this section we study the effect of increasing the max RF without changing the number of the CNN parameters. 
In Section~\ref{sub:sec:maxrf:generalization}, we showed the effect of changing the Max RF of a CNN, on both the training and the testing loss, by changing the filter sizes in CNN layers.
One possible side effect when the Max RF increases in this method is that the number of parameters of the network increases. 
In contrast to this approach, We can increase the Max RF by changing the strides of the CNN layers. 
In practice, It is common \khaled{cite} to use Max pooling layers of size $2 x 2$ with a stride of $2 $. 
Pooling layers does not affect the number of parameters of a model,  as they are down sampling operators with no parameters.
Equation~\ref{eq:calc_maxrf} shows that a layer with a stride of $2 $ doubles the Max RF of all the following layers. 
Hence, we can add or remove pooling layer from the network to change its RF without changing the number of its parameters. 
Although using this technique, we can control the Max RF without changing the number of parameters in the model, this approach has less flexibility in the level of controlling Max RF.
Figure~\ref{fig:train_vs_test_by_maxrf_pooling} Shows a similar pattern to Figure~\ref{fig:train_vs_test_by_maxrf}.



\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{figs/test_vs_train_loss_by_maxrf_dcase18_pooling.png}
\caption{Comparing the training loss vs the testing loss of CP\_ResNet with different Max RF. The increase of the testing loss with larger Max RF indicates overfitting. Note that we use Mix-up for the training data.\khaled{add ERF maybe}}
\label{fig:train_vs_test_by_maxrf_pooling}
\end{figure}


==> ommited_a2_dilated_cnns.tex <==
\label{app:dilated}
\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_dilated_loss.pdf}
\caption{Testing loss of CP\_ResNet with some dilated convolution layers. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $57 \times 57$ to $345 \times 345$}
\label{fig:dcase18:dilated:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_dilated_acc.pdf}
\caption{Testing accuracy CP\_ResNet with some dilated convolution layers. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $57 \times 57$ to $345 \times 345$}
\label{fig:dcase18:dilated:acc}
\end{figure}

In this section, we will show the results of dilated CNNs on an acoustic scene classification task using the DCASE 2018 dataset (Section~\ref{sec:tasks_datasets}). 
We start the experiment with variants of CP\_ResNet with a Max RF ranging from $55 \time 55$ pixels to $199 \time 199$ (corresponding $\psi$ from $3$ to $9$). 
We then change the convolution of different layers (in different experiments) to a dilated convolutional operator with $d=2$. 
We then calculate the Max RF by substituting $k_n$ with $ d(k_n-1)+1$ in Equation~\eqref{eq:calc_maxrf} as explained in Section~\ref{sec:sub:dilated:cnn}. Figures~\ref{fig:dcase18:dilated:loss} and~\ref{fig:dcase18:dilated:acc} shows the testing loss and accuracy for these networks. 
The figures show that the dilated CNNs follow a similar a pattern to previous CNN results. 


==> ommited_a3_grouped_cnns.tex <==
\label{app:grouped}

\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_grouped_loss.pdf}
\caption{Testing loss of CP\_ResNet with grouped convolution layers. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $551 \times 551$}
\label{fig:dcase18:grouped:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_grouped_acc.pdf}
\caption{Testing accuracy CP\_ResNet with grouped convolution layers. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $551 \times 551$}
\label{fig:dcase18:grouped:acc}
\end{figure}

In this section, we will show the results of grouped CNNs on an acoustic scene classification task using the DCASE 2018 dataset (Section~\ref{sec:tasks_datasets}). Figures~\ref{fig:dcase18:grouped:loss} and~\ref{fig:dcase18:grouped:acc} show the loss and accuracy of CP\_ResNet (Section~\ref{sec:control_max_rf}) with  grouped convolutional layers. We show the results of different variants with different number of groups. The figures shows that grouped convolutional networks follows a similar pattern as expected and explained in Section~\ref{sec:control_max_rf}.
\khaled{The figures shows the mean of multiple runs, we didn't plot the variance for visibility.}



==> ommited_a4_dense_cnns.tex <==
\label{app:densenet:asc}
\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_dense_loss.pdf}
\caption{Testing loss of CP\_Dense Illustrating skip connections. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $551 \times 551$}
\label{fig:dcase18:dense:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase_dense_acc.pdf}
\caption{Testing accuracy of CP\_Dense Illustrating skip connections. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $551 \times 551$}
\label{fig:dcase18:dense:acc}
\end{figure}

In this section, we will show the results of CP\_DenseNet (Section~\ref{sec:control_maxrf:densenet}) variants on an acoustic scene classification task using the DCASE 2018 dataset (Section~\ref{sec:tasks_datasets}).


Figures~\ref{fig:dcase18:dense:loss} and~\ref{fig:dcase18:dense:acc} show the loss and accuracy of CP\_DenseNet. We show the results of different variants with different number of growth rate. The figures shows that DenseNet networks (CNNs with skip connections) follows a similar pattern as expected and explained in Section~\ref{sec:control_max_rf}.

The figures show having a growth rate 32, restricts the network performance compared to a growth-rate of 64 and 128 in the optimal Max RF range. While the networks have a comparable performance in larger RF ranges. 

==> ommited_a5_further_asc.tex <==
%"figs_dcase17_loss.pdf" "figs_dcase17_acc.pdf"
\label{app:further:asc:dcase}
\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase19_loss.pdf}
\caption{Testing loss of CP\_ResNet on DCASE 2019 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase19:resnet:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase19_acc.pdf}
\caption{Testing accuracy of CP\_ResNet  on DCASE 2019 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase19:resnet:acc}
\end{figure}

\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/figs_dcase17_loss.pdf}
\caption{Testing loss of CP\_ResNet  on DCASE 2017 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase17:resnet:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/figs_dcase17_acc.pdf}
\caption{Testing accuracy of CP\_ResNet on DCASE 2017 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase17:resnet:acc}
\end{figure}

\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/figs_dcase16_loss.pdf}
\caption{Testing loss of CP\_ResNet  on DCASE 2016 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase16:resnet:loss}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/figs_dcase16_acc.pdf}
\caption{Testing accuracy of CP\_ResNet on DCASE 2016 ASC Dataset. The Max RF size of the network over both time and frequency dimensions (x-axis) is ranging from $23 \times 23$ to $350 \times 350$}
\label{fig:dcase16:resnet:acc}
\end{figure}


\begin{figure}[h]
%fa_analysis-2d_dcase_freq_rime.ipynb
\centering
\includegraphics[width=3.5in]{figs/dcase18_2d_loss_train.pdf}
\caption{Training loss of different variants of CP\_ResNet with changing Max-RF over time (x-axis) and frequency (y-axis), the variants has a Max-RF ranging from $23 \times 23$ to $551 \times 551$}
\label{fig:dcase18:2d_loss:time_freq:train}
\end{figure}


In this Section, we present the results of CP\_ResNet on different acoustic scene classification datasets, DCASE 2019 ASC in Figures~\ref{fig:dcase19:resnet:loss} and ~\ref{fig:dcase19:resnet:acc}, DCASE 2017  ASC in Figures~\ref{fig:dcase17:resnet:loss} and ~\ref{fig:dcase17:resnet:acc}, DCASE 2016 ASC in Figures~\ref{fig:dcase16:resnet:loss} and ~\ref{fig:dcase16:resnet:acc}. The figures show the network follows  a similar pattern on all the datasets.

Figure~\ref{fig:dcase18:2d_loss:time_freq:train} shows the training loss of CP\_ResNet on DCASE 2018. The figure shows that increasing the Max RF of the CNN on either of the dimensions, increases it's capability to fit the training data. However, by comparing to Figure~\ref{fig:dcase18:2d_loss:time_freq}, we see that bigger RF correlated with a higher testing loss.

==> unused_text.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=2.5in]{figs/speach_resnet.png}
\caption{The Effective Receptive Field (ERF) of a Deep ResNet trained on a single class speech tagging task.
\gerhard{The max RF is indicated by the ... box. OR: The max RF corresponds to the entire spectrogram patch shown. [Is this correct??]}}
\label{fig:erf_speech}
\end{figure}


\subsection{Illustration: The Effective Receptive Field for a Speech Tagging Task }
\label{sec:motivation:erf_speach}
% \hamid{I find this section a little bit off the story line of the paper.
% We explain that we focus on 3 tasks, but all of the sudden, we come up with a 4th task, as motivation.
% It is a bit strange.
% Either we need to very well motivate why we chose speech tagging for motivation (and why not ASC or other tasks?);
% or we need to introduce it as the 4th task, which then needs to be properly evaluated.
% Another option is to show some ERF from other tasks (e.g, ASC), which makes the most sense.
% % It may as well save some space here.
% It seems the next section has already some examples for ASC, we could skip it here altogether.
% }
% \khaled{explicitly this a toy example, STRF related}

To illustrate the ERF on a `toy' problem, we train a CNN to perform a simple speech tagging task.
The objective is to tag an audio clip by whether a speech signal is present in the audio. 
For the experiment, we use the DCASE-2018 task 4 dataset~\cite{serizel2018_dcase17_task4}. 
Since in our task, we only predict the overall tag, and not the location of the event, 
% we use only the weak labels since we are dealing with an audio tagging task.
we use only the weakly labeled part of the training set~\cite{serizel2018_dcase17_task4}, which contains
1578 audio clips with a duration of 10 seconds each.
% , where each has a length of 10 seconds. 
We use the testing part of the development set for testing, which consists of 288 audio clips of 10 seconds. 
We train a ResNet with a large maximum receptive field of $913x913$ pixels to reach $92.4\%$ accuracy on the testing set. 
%We consider speech tagging a simple problem for CNNs compared to multi-class problems we discuss later in this paper. 
%We study the ERF of the trained network in Figure~\ref{fig:erf_speech}. 

The ERF of the trained model for the speech detection task is visualised in Figure~\ref{fig:erf_speech}. We see the ERF is much smaller than the max RF.
The trained model learned to ignore large ranges of frequencies, and focus mostly on a narrow frequency range of the input spectrogram. 
This is consistent with the characteristics of the task, since speech information is expected to be in the narrow frequency range.% , i.e. effective receptive field of the network. 


In the case of more difficult tasks, and knowing the capability of deep neural networks to fit even random data or labels~\cite{rethinkinggeneralizationZhangBHRV17}, this raises the question of whether larger RFs encourages CNNs to base their predictions on learned patterns in the training set that don't generalize to unseen test data. 
We look at this in the next section, using a more challenging
multi-class classification task. 







\subsection{Increasing The Max RF with Pooling}
\label{app:maxrf:traintest:pooling}

In this section we study the effect of increasing the max RF without changing the number of the CNN parameters. 
In Section~\ref{sub:sec:maxrf:generalization}, we showed the effect of changing the Max RF of a CNN, on both the training and the testing loss, by changing the filter sizes in CNN layers.
One possible side effect when the Max RF increases in this method is that the number of parameters of the network increases. 
In contrast to this approach, We can increase the Max RF by changing the strides of the CNN layers. 
In practice, It is common \khaled{cite} to use Max pooling layers of size $2 x 2$ with a stride of $2 $. 
Pooling layers does not affect the number of parameters of a model,  as they are down sampling operators with no parameters.
Equation~\ref{eq:calc_maxrf} shows that a layer with a stride of $2 $ doubles the Max RF of all the following layers. 
Hence, we can add or remove pooling layer from the network to change its RF without changing the number of its parameters. 
Although using this technique, we can control the Max RF without changing the number of parameters in the model, this approach has less flexibility in the level of controlling Max RF.
Figure~\ref{fig:train_vs_test_by_maxrf_pooling} Shows a similar pattern to Figure~\ref{fig:train_vs_test_by_maxrf}.








%%
% THis Section is rewritten and merged with the previous section

%%

% \subsection{An Objective Measure for the Effective RF in CNNs }
% \label{sec:rf_cnns:erf:measure}

% In Section~\ref{sec:rf_cnns:erf}, we explained an approach for visualizing the ERF of CNNs. 
% In this section, we introduce a new method to objectively measure the size of the ERF, in the time and the frequency dimensions.
% %  
% We will use these ERF size estimates in Sections~\ref{sec:control_erf} to study a proposed method to control the ERF without altering a CNN architecture, and in Section~\ref{sec:result_erf} where we investigate the size of the ERF on the performance of CNNs.



% Our approach for objective measurement of ERF is similar in nature to~\cite{luoUnderstandingEffectiveReceptive2016}.
% However, in~\cite{luoUnderstandingEffectiveReceptive2016}, Luo et al. propose an approach to find  ``impactful regions'' in the input of the model, while we propose an objective numerical measure for this impactful region.
% \gerhard{What are "impactful regions" in your case? do you actually compute "regions"? or just importance values for individual input pixels (which you then model with a Gaussian (see below))? (remember: a "region" is a thing, with a boundary.) If it is importance values for pixels: is your method here different from your method in IV.B? in what way, and why? And finally: I understand you do this over a whole data set and average the values? - if so, this should also be clearly, explicity said (once again). }
% We propagate a gradient signal from the last layer of the network that still has the spatial information about time dimension (before global pooling), back to the input.
% The impactful regions of the input are then calculated based on this gradient.
% In Figure~\ref{fig:erf_visual} we visualise these impactful regions, averaged over the test set of the DCASE-18 acoustic scenes dataset.


% Although this method allows us to visualise the regions that a model focuses on, it can not be used for an objective comparison and evaluation between different models.
% To tackle this problem, we propose to quantify the effective receptive field size of a CNN by two scalars $E_t$ and $E_f$, indicating the effective receptive field over the time and frequency dimension respectively.% We detail these measurements in the following.

% Luo et al.~\cite{luoUnderstandingEffectiveReceptive2016} showed that the distribution of the impactful regions \gerhard{again: "regions" follow a distribution? or what exactly are the things that give a Gaussian: pixels?}
% inside the maximum receptive field follows a Gaussian distribution. 
% In other words, they show that the effective receptive field is distributed as an asymptotic Gaussian. 
% Based on this assumption, we estimate the standard deviation $\sigma_t$,$\sigma_f$ of the ERF on the time or frequency dimension. We use $E= 4 * \sigma$ as an estimate of the effective receptive field size, since $Pr(\mu -2\sigma \leq X\leq \mu +2\sigma ) \approx 0.9545$. Therefore, the region of length $E= 4 * \sigma$ around the center of the ERF contains $0.9545$ of the impactful pixels (Gaussian assumption). In practice, we calculate the centers $\mu_t$, $\mu_f$ and std deviations $\sigma_t$, $\sigma_f$ as shown in Equations~\eqref{eq:calc_erf_center}. \khaled{@Gerhard: is this explanation suitable?}
% \gerhard{No, I don't get it. What is $g()?$ what is the dot in $x . g(x)$? is this supposed to be multiplication? What are you summing over?}

% \begin{align}    
% \nonumber \mu_x &= \frac{ \sum x . g(x) }{\sum g(x)} \\
% \sigma_x &= \sqrt{ \frac{ \sum g(x)(x - \mu_x)^2 }{\sum g(x)}}
% \label{eq:calc_erf_center}
% \end{align}
% where $x$ is either the time $t$ or frequency $f$ dimension while $\mu_x$ is the center on the $x$ dimension.

% Figure~\ref{fig:erf_visual} visualizes the ERF, the maximum RF, and our estimates $E_t$ and $E_f$ for a ResNet with a Maximum RF of  $241 \times 241$  trained on DCASE-18 ASC dataset~\cite{MesarosDCASE2018T1}. We see that the ERF has a smaller spread compared to the maximum RF. We can also see in this ASC task with 10 classes that ERF has a Gaussian shape on both dimensions.
